Temporal CSI Correlation in Mixed RF/FSO Cooperative Relaying Systems Under Joint Effects of HPA Nonlinearities and IQ Imbalance

In this paper, we present the performance analysis of mixed RF/FSO system with multiple relays. To select the best relay, we adopt partial relay selection with outdated CSI wherein we investigate the effect of the temporal correlation of the channels. Unlike the vast majority of work, we introduce the impairments to the relays and the destination and we compare the performance against conventional RF relaying systems. We further derive the expressions of the outage probability and the ergodic capacity as well as the bounds to unpack engineering insights into the system robustness.

==> performance.tex <==
\section{Performance Analysis}
In this section, we present the analysis of the OP, the BER and the EC. We will show that the OP and BER are limited by irreducible floors and the EC is finite and saturated by a ceiling at the high SNRs values. The floors and the ceiling are certainly caused by the hardware impairments originating from the relays and the destination.
\subsection{Outage Probability Analysis}
The outage probability is defined as the probability that the end-to-end SNDR falls below a given outage threshold $\gamma_{\text{th}}$. It can be written as follows
\begin{equation}
P_{\text{out}}(\gamma_{\text{th}}) \delequal \text{Pr}[\gamma_{\text{e2e}} < \gamma_{\text{th}}],
\end{equation}
where \text{Pr($\cdot$)} is the probability notation. The analytical expression of the SNDR given by Eq.~(21) should be placed in Eq.~(18). After some algebraic manipulations, the OP can be expressed by Eq.~(22). Note that the CDF $F_{\gamma_{1(m)}}$ is defined only if $1 - \text{ILR}\gamma_{\text{th}} > 0$, otherwise it is equal to a unity.
The term $\kappa$ is the ratio between the received SNR and the average transmitted SNDR at the relay which is given by
\begin{equation}
\kappa = 1 + \frac{\sigma_d^2}{\delta^2G^2\sigma_0^2},
\end{equation}
Note that the OP is equal to Eq.~(24) for $\gamma_{\text{th}} < \frac{1}{\text{ILR}}$, otherwise, it is equal to a unity.\\
Since the expression of the outage probability involves complex function such as the Meijer-G function, we need to derive an asymptotic high SNR expression to unpack engineering insights about the system gain. Given that the outage performance saturates at high SNR by the outage floor caused by the hardware impairments, it is trivial to conclude that the diversity gain $G_d$ is equal to zero. For an ideal hardware and after expanding the Meijer-G function at high SNR using \cite[Eq.~(07.34.06.0001.01)]{24}, it can be shown that the diversity gain is given by
\begin{equation}
G_d = \min\left(1,~\frac{\alpha}{2},~\frac{\beta}{2}\right),  
\end{equation}
\subsection{Average Bit Error Rate}
The BER can be expressed as follows
\begin{equation}
\overline{P_e} = \frac{q^p}{2\Gamma(p)}\int\limits_{0}^{\infty}\gamma^{p-1}e^{-q\gamma}~F_{\gamma_{\text{e2e}}}(\gamma)~d\gamma,  
\end{equation}
where $F_{\gamma_{\text{e2e}}}(\cdot)$ is the CDF of $\gamma_{\text{e2e}}$, $p$ and $q$ are the parameters that indicate the modulation format, respectively. As we mentioned earlier, the mathematical terms related to the impairments render the integral calculus very complex. As a result, deriving a closed-form of the BER is not possible. In this case, a numerical integration is required. Note that a floor occurs at high SNRs values which prevents the BER from converging to zero. This floor will be shown graphically later in the section of numerical results.
\newpage
\begin{strip}
\noindent\rule{18.5cm}{1pt}
\vspace*{0.5cm}
\begin{equation}
\gamma_{e2e} = \frac{\gamma_{1(m)}\gamma_{2(m)}}{\text{ILR}\gamma_{1(m)}\gamma_{2(m)}+(1+\text{ILR})\kappa\gamma_{2(m)}+(1+\text{ILR})(\e{\gamma_{1(m)}} + \kappa)},
\end{equation}
\noindent\rule{18.5cm}{1pt}
%\vspace*{0.5cm}
\begin{equation}
\begin{split}
P_{\text{out}}(\gamma_{\text{th}}) =& 1 - \frac{2^{\alpha+\beta-2}}{\pi\Gamma(\alpha)\Gamma(\beta)}m{N \choose m} \sum_{n=0}^{m-1} {m-1 \choose n}\frac{(-1)^n}{N-m+n+1}
\exp\left(-\frac{(N-m+n+1)\kappa(1+\text{ILR})\gamma_{\text{th}}}{((N-m+n)(1-\rho)+1)(1-\text{ILR}\gamma_{\text{th}})\overline{\gamma}_1}\right)\\&
\times~\MeijerG[\Bigg]{5}{0}{0}{5}{-}{\frac{\alpha}{2}, \frac{\alpha+1}{2}, \frac{\beta}{2}, \frac{\beta+1}{2}, 0}{\frac{(\alpha\beta)^2(\e{\gamma_{1(m)}}+\kappa)(N-m+n+1)\gamma_{\text{th}}}{16((N-m+n)(1-\rho)+1)(1-\text{ILR}\gamma_{\text{th}})\overline{\gamma}_1 \overline{\gamma}_2}},
\end{split}
\end{equation}
%\vspace*{0.5cm}
\noindent\rule{18.5cm}{1pt}
\end{strip}
\vspace*{-1cm}
\subsection{Ergodic Capacity}
The ergodic capacity, expressed in bit/s/Hz, is defined as the  maximum error-free data transferred by the channel of the system. It can be written as follows
\begin{equation}
\overline{C} \delequal \frac{1}{2}\e{\log_{2}(1+\gamma_{\text{e2e}})},
\end{equation}
The capacity can be calculated by deriving the PDF of the SNDR. However, an exact closed-form of Eq.~(26) is very difficult due to the mathmatical terms related to the impairments. To evaluate the system capacity, we should refer to the numerical integration.\\
In spite of the difficulty to calculate an exact closed-form of the EC, we can derive a simpler expression by referring to the approximation given by \cite[Eq.~(27)]{22}
\begin{equation}
\e{\log_2\left(1 + \frac{\psi}{\varphi}\right)} \approx \log_2\left(1+\frac{\e{\psi}}{\e{\varphi}} \right),
\end{equation}
For high SNR values, the SNDR converges to $\gamma^*$ defined by
\begin{equation}
\lim_{\overline{\gamma}_1,\overline{\gamma}_2\to\infty}\gamma_{\text{e2e}} = \frac{1}{\frac{(1+\text{ILR})\xi}{\delta}-1} = \gamma^*,
\end{equation}
\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\begin{cor}
Suppose that $\overline{\gamma}_1$ and $\overline{\gamma}_2$ converge to infinity and the electrical and optical channels are independent, the ergodic capacity converges to a capacity ceiling defined by
\begin{equation}
\overline{C}^* = \frac{1}{2}\log_2(1+\gamma^*), 
\end{equation}
\end{cor}
\begin{proof}
Since the SNDR converges to $\gamma^*$ as the average SNRs of the first and second hop largely increase, the dominated convergence theorem allows to move the limit inside the logarithm function.
\end{proof}
If the relaying system is linear, i.e, the system is only impaired by IQ imbalance, the SNDR and the average capacity are saturated at the high SNR regime as follows
\begin{equation}
\gamma^* = \frac{1}{\text{ILR}},~~\overline{C}^{*} = \frac{1}{2}\log_2\left(1+\frac{1}{\text{ILR}}\right),
\end{equation}
To characterize the EC, it is possible to derive the expression of the upper bound stated by the following theorem.
\newtheorem{theorem}{Theorem}
\begin{theorem}
For asymmetric (Rayleigh/Gamma-Gamma) fading channels, the ergodic capacity $\overline{C}$ for non-ideal hardware is upper bounded by
\begin{equation}
    \overline{C} \leq \frac{1}{2}\log_{2}\left(1 + \frac{\mathcal{J}}{\text{ILR}~\mathcal{J} + 1}\right)
\end{equation}
\end{theorem}
where $\mathcal{J}$ is given by
\begin{equation}
\begin{split}
 \mathcal{J} = \e{\frac{\gamma_{1(m)}\gamma_{2(m)}}{\text{ILR}\gamma_{2(m)} + \tau }},
 \end{split}
\end{equation}
where $\tau = (1+\text{ILR})\kappa\gamma_{2(m)}+(1+\text{ILR})(\e{\gamma_{1(m)}} + \kappa)$.\\
After some mathematical manipulations, $\mathcal{J}$ is given by
\begin{equation}
\begin{split}
&\mathcal{J} = \ddfrac{m{N \choose m}(\alpha\beta)^\frac{\alpha + \beta}{2}\left( \frac{\e{\gamma_{1(m)}} + \kappa}{\kappa}\right)^\frac{\alpha+\beta}{4}}{2\pi(1+\text{ILR})\kappa\Gamma(\alpha)\Gamma(\beta)\overline{\gamma}_2^\frac{\alpha+\beta}{4}}\\&~
\times \sum_{n=0}^{m-1} {m-1 \choose n}\frac{(-1)^m((N-m+n)(1-\rho)+1)\overline{\gamma}_1}{(N-m+n+1)^2}\\&
\times~\MeijerG[\Bigg]{5}{1}{1}{5}{\kappa_0}{\kappa_1}
{\frac{(\alpha\beta)^2(\e{\gamma_{1(m)}}+\kappa)}{16\kappa\overline{\gamma}_2}},
\end{split}
\end{equation}
where $\kappa_0, \kappa_1$ are given by
\begin{equation}
\begin{split}
&\kappa_0 = -\frac{\alpha + \beta}{4},\\&
\kappa_1 = \left[\frac{\alpha - \beta}{4}, \frac{\alpha - \beta + 2}{4}, \frac{\beta - \alpha}{4}, \frac{\beta - \alpha +2 }{4},-\frac{\alpha + \beta}{4}\right],
\end{split}
\end{equation}
